Towards Federated Domain Unlearning: Verification Methodologies and Challenges

Federated Learning (FL) has evolved as a powerful tool for collaborative model training across multiple entities, ensuring data privacy in sensitive sectors such as healthcare and finance. However, the introduction of the Right to Be Forgotten (RTBF) poses new challenges, necessitating federated unlearning to delete data without full model retraining. Traditional FL unlearning methods, not originally designed with domain specificity in mind, inadequately address the complexities of multi-domain scenarios, often affecting the accuracy of models in non-targeted domains or leading to uniform forgetting across all domains. Our work presents the first comprehensive empirical study on Federated Domain Unlearning, analyzing the characteristics and challenges of current techniques in multi-domain contexts. We uncover that these methods falter, particularly because they neglect the nuanced influences of domain-specific data, which can lead to significant performance degradation and inaccurate model behavior. Our findings reveal that unlearning disproportionately affects the model's deeper layers, erasing critical representational subspaces acquired during earlier training phases. In response, we propose novel evaluation methodologies tailored for Federated Domain Unlearning, aiming to accurately assess and verify domain-specific data erasure without compromising the model's overall integrity and performance. This investigation not only highlights the urgent need for domain-centric unlearning strategies in FL but also sets a new precedent for evaluating and implementing these techniques effectively.

==> Digits_test_acc.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}



\begin{table*}[]
\caption{
In the context of the Domain-Digits dataset, after unlearning a specific domain using various methods, we evaluated the training and testing accuracy for each domain.}
\renewcommand{\arraystretch}{1.4}
\resizebox{\textwidth}{!}{%

\begin{tabular}{cccccccccccc}
\hline
\multicolumn{2}{c}{\multirow{1}{*}{\textbf{Domain-Digits}}} &
  \multicolumn{5}{c}{\multirow{1}{*}{\textbf{Train  ACC  For All  Domain}}} &
  \multicolumn{5}{c}{\multirow{1}{*}{\textbf{Test  ACC  For All  Domain}}} \\ 
% \multicolumn{2}{c}{} &
%   \multicolumn{5}{c}{} &
%   \multicolumn{5}{c}{} \\ 
\hline
\textbf{Unlearn Domain} &
  \textbf{Method} &
  \textbf{MNIST} &
  \textbf{SVHN} &
  \textbf{USPS} &
  \textbf{SynthDigits} &
  \textbf{MNIST-M} &
  \textbf{MNIST} &
  \textbf{SVHN} &
  \textbf{USPS} &
  \textbf{SynthDigits} &
  \textbf{MNIST-M} \\ \hline
\textbf{/} &
  Full learn &
  99.99 &
  94.15 &
  98.62 &
  98.67 &
  98.82 &
  98.91 &
  83.36 &
  97.42 &
  93.57 &
  90.40 \\ \hline
\multirow{5}{*}{\textbf{MNIST}} &
  Retrain &
  97.82±0.08 &
  97.82±0.11 &
  99.09±0.03 &
  99.74±0.07 &
  98.66±0.17 &
  97.83±0.21 &
  85.20±0.21 &
  97.42±0.02 &
  94.78±0.08 &
  89.35±0.14 \\
 &
  BL1 Repaid Retrain &
  96.83±0.02 &
  92.82±0.13 &
  99.50±0.04 &
  99.69±0.06 &
  95.91±0.12 &
  96.80±0.01 &
  80.30±0.08 &
  97.90±0.05 &
  92.64±0.11 &
  82.14±0.19 \\
 &
  BL2 FedEraser &
  95.21±0.12 &
  81.04±0.23 &
  95.40±0.09 &
  90.97±0.15 &
  83.52±0.23 &
  95.08±0.23 &
  76.96±0.40 &
  95.22±0.27 &
  88.38±0.11 &
  80.57±0.12 \\
 &
  BL3 Increase Loss &
  96.84±0.09 &
  97.06±0.17 &
  99.41±0.04 &
  99.93±0.03 &
  99.61±0.11 &
  95.96±0.11 &
  84.32±0.05 &
  97.8±0.02 &
  94.46±0.04 &
  90.19±0.10 \\
 &
  BL4 Class Pruning &
  98.66±0.01 &
  97.15±0.50 &
  99.45±0.01 &
  99.96±0.00 &
  99.81±0.12 &
  98.14±0.02 &
  84.48±0.08 &
  97.8±0.05 &
  94.66±0.01 &
  90.46±0.35 \\  \hline
\multirow{5}{*}{\textbf{SVHN}} &
  Retrain &
  100.00±0.00 &
  67.84±0.30 &
  98.83±0.10 &
  98.60±0.48 &
  99.26±0.20 &
  99.09±0.05 &
  67.48±0.58 &
  97.63±0.11 &
  91.49±0.56 &
  92.28±0.28 \\
 &
  BL1 Repaid Retrain &
  100.00±0.00 &
  62.38±0.26 &
  98.92±0.03 &
  97.69±0.51 &
  95.94±0.56 &
  98.79±0.00 &
  62.55±0.74 &
  97.42±0.00 &
  89.07±0.22 &
  85.76±0.17 \\
 &
  BL2 FedEraser &
  99.95±0.20 &
  63.57±0.54 &
  98.57±0.27 &
  95.86±0.63 &
  97.45±0.41 &
  98.94±0.33 &
  63.41±0.60 &
  97.26±0.21 &
  89.42±0.43 &
  90.54±0.45 \\
 &
  BL3 Increase Loss &
  99.97±0.02 &
  73.42±0.48 &
  99.37±0.02 &
  99.72±0.11 &
  99.78±0.03 &
  98.99±0.03 &
  70.12±0.58 &
  98.01±0.05 &
  93.59±0.09 &
  92.36±0.14 \\
 &
  BL4 Class Pruning &
  99.99±0.00 &
  73.45±0.39 &
  99.26±0.05 &
  99.09±0.10 &
  99.92±0.01 &
  98.99±0.00 &
  70.82±0.97 &
  97.85±0.02 &
  92.54±0.37 &
  92.65±0.19 \\  \hline
\multirow{5}{*}{\textbf{USPS}} &
  Retrain &
  99.89±0.01 &
  93.92±0.24 &
  89.33±0.01 &
  99.54±0.25 &
  99.60±0.12 &
  98.49±0.07 &
  83.35±0.01 &
  89.30±0.03 &
  94.05±0.17 &
  91.21±0.15 \\
 &
  BL1 Repaid Retrain &
  99.91±0.00 &
  87.24±0.28 &
  88.94±0.02 &
  99.10±0.09 &
  98.82±0.16 &
  98.49±0.12 &
  78.73±0.04 &
  88.87±0.15 &
  91.68±0.02 &
  86.89±0.04 \\
 &
  BL2 FedEraser &
  98.37±0.10 &
  79.35±0.19 &
  87.95±0.25 &
  89.93±0.27 &
  89.10±0.18 &
  97.64±0.15 &
  75.94±021 &
  86.88±0.11 &
  87.62±0.21 &
  85.56±0.15 \\
 &
  BL3 Increase Loss &
  99.88±0.00 &
  95.68±0.03 &
  82.83±0.04 &
  99.78±0.01 &
  99.65±0.01 &
  98.51±0.21 &
  83.93±0.11 &
  82.80±0.05 &
  94.24±0.03 &
  90.79±0.06 \\
 &
  BL4 Class Pruning &
  99.93±0.00 &
  95.7±0.02 &
  91.87±0.02 &
  99.93±0.06 &
  99.87±0.02 &
  98.74±0.05 &
  84.40±0.02 &
  91.83±0.06 &
  94.55±0.11 &
  91.58±0.08 \\ \hline
\multirow{5}{*}{\textbf{SynthDigits}} &
  Retrain &
  99.96±0.00 &
  87.21±0.34 &
  99.31±0.27 &
  82.31±0.61 &
  99.33±0.02 &
  98.90±0.02 &
  76.51±0.59 &
  97.31±0.17 &
  82.50±0.65 &
  91.54±0.18 \\ 
 &
  BL1 Repaid Retrain &
  99.97±0.00 &
  80.22±0.79 &
  98.39±0.10 &
  77.78±0.27 &
  97.88±0.32 &
  98.64±0.09 &
  71.22±0.82 &
  96.88±0.17 &
  77.98±0.12 &
  87.14±0.27 \\
 &
  BL2 FedEraser &
  99.26±0.02 &
  77.36±0.71 &
  95.66±0.23 &
  77.75±0.27 &
  93.22±0.30 &
  98.14±0.01 &
  71.72±0.81 &
  94.57±0.42 &
  78.15±0.32 &
  87.49±0.13 \\
 &
  BL3 Increase Loss &
  100.00±0.00 &
  91.41±0.68 &
  99.22±0.03 &
  85.49±0.11 &
  99.76±0.02 &
  98.82±0.05 &
  79.04±0.27 &
  97.69±0.06 &
  84.3±0.17 &
  91.77±0.05 \\
 &
  BL4 Class Pruning &
  100.00±0.00 &
  93.12±0.12 &
  99.58±0.04 &
  87.81±0.05 &
  99.89±0.03 &
  98.96±0.00 &
  80.59±0.10 &
  98.06±0.05 &
  86.88±0.16 &
  91.59±0.19 \\ \hline
\multirow{5}{*}{\textbf{MNIST-M}} &
  Retrain &
  99.87±0.00 &
  94.94±0.85 &
  99.57±0.01 &
  99.78±0.07 &
  69.9±0.09 &
  98.39±0.02 &
  84.21±0.62 &
  98.49±0.05 &
  94.73±0.09 &
  70.35±0.10 \\ 
 &
  BL1 Repaid Retrain &
  99.72±0.01 &
  89.14±0.39 &
  99.39±0.01 &
  99.37±0.02 &
  65.84±0.11 &
  97.90±0.02 &
  80.40±0.11 &
  97.58±0.00 &
  93.13±0.02 &
  65.49±0.07 \\
 &
  BL2 FedEraser &
  99.50±0.22 &
  92.22±1.30 &
  99.26±0.21 &
  99.13±0.64 &
  68.73±0.25 &
  97.75±0.09 &
  82.79±0.71 &
  98.12±0.58 &
  94.16±0.21 &
  68.76±0.39 \\
 &
  BL3 Increase Loss &
  99.30±0.03 &
  96.88±0.04 &
  99.56±0.09 &
  99.91±0.00 &
  72.60±0.04 &
  97.48±0.04 &
  84.30±0.02 &
  98.28±0.05 &
  95.12±0.02 &
  70.31±0.03 \\
 &
  BL4 Class Pruning &
  99.92±0.00 &
  96.57±0.03 &
  99.84±0.00 &
  99.95±0.00 &
  77.60±0.01 &
  98.55±0.02 &
  84.84±0.10 &
  98.23±0.07 &
  95.33±0.17 &
  75.22±0.21   \\ \hline
\end{tabular}

}
\end{table*}

==> DomainNet_test_acc.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\begin{tabular}{cl|cccccc}
%\hline
\multicolumn{2}{c|}{\multirow{2}{*}{\textbf{DomainNet}}} &
  \multicolumn{6}{c}{\multirow{2}{*}{\textbf{Test  ACC  For All  Domain}}} \\
\multicolumn{2}{c|}{} &
  \multicolumn{6}{c}{} \\ \hline
\multicolumn{1}{c|}{\textbf{Unlearn Domain}} &
  \textbf{BaseLine} &
  \multicolumn{1}{c|}{\textbf{Clipart}} &
  \multicolumn{1}{c|}{\textbf{Infograph}} &
  \multicolumn{1}{c|}{\textbf{Painting}} &
  \multicolumn{1}{l|}{\textbf{Quickdraw}} &
  \multicolumn{1}{c|}{\textbf{Real}} &
  \textbf{Sketch} \\ \hline
\multicolumn{1}{c|}{\textbf{/}} &
  Full learn &
  \multicolumn{1}{c|}{86.69} &
  \multicolumn{1}{c|}{49.01} &
  \multicolumn{1}{c|}{78.35} &
  \multicolumn{1}{c|}{76.6} &
  \multicolumn{1}{c|}{79.62} &
  84.48 \\ \hline
\multicolumn{1}{c|}{\multirow{5}{*}{\textbf{Clipart}}} &
  BL0 Retrain &
  \multicolumn{1}{c|}{72.43} &
  \multicolumn{1}{c|}{45.97} &
  \multicolumn{1}{c|}{77.54} &
  \multicolumn{1}{c|}{72.4} &
  \multicolumn{1}{c|}{78.88} &
  81.05 \\ \cline{2-8} 
\multicolumn{1}{c|}{} &
  BL1 Repaid Retrain &
  \multicolumn{1}{c|}{56.46} &
  \multicolumn{1}{c|}{32.27} &
  \multicolumn{1}{c|}{54.28} &
  \multicolumn{1}{c|}{63.1} &
  \multicolumn{1}{c|}{61.54} &
  50.18 \\ \cline{2-8} 
\multicolumn{1}{c|}{} &
  BL2 FedEraser &
  \multicolumn{1}{c|}{71.48} &
  \multicolumn{1}{c|}{40.64} &
  \multicolumn{1}{c|}{72.54} &
  \multicolumn{1}{c|}{66.5} &
  \multicolumn{1}{c|}{74.94} &
  77.98 \\ \cline{2-8} 
\multicolumn{1}{c|}{} &
  BL3 Increase Loss &
  \multicolumn{1}{c|}{78.14} &
  \multicolumn{1}{c|}{45.51} &
  \multicolumn{1}{c|}{80.45} &
  \multicolumn{1}{c|}{72.8} &
  \multicolumn{1}{c|}{79.38} &
  86.1 \\ \cline{2-8} 
\multicolumn{1}{c|}{} &
  Bl4 Class Pruning &
  \multicolumn{1}{c|}{77.76} &
  \multicolumn{1}{c|}{45.05} &
  \multicolumn{1}{c|}{79.16} &
  \multicolumn{1}{c|}{75} &
  \multicolumn{1}{c|}{80.12} &
  84.48 \\ \hline
\multicolumn{1}{c|}{\multirow{5}{*}{\textbf{Infograph}}} &
  BL0 Retrain &
  \multicolumn{1}{c|}{86.5} &
  \multicolumn{1}{c|}{37.14} &
  \multicolumn{1}{c|}{79.32} &
  \multicolumn{1}{c|}{76.9} &
  \multicolumn{1}{c|}{80.44} &
  86.1 \\ \cline{2-8} 
\multicolumn{1}{c|}{} &
  BL1 Repaid Retrain &
  \multicolumn{1}{c|}{68.82} &
  \multicolumn{1}{c|}{28.46} &
  \multicolumn{1}{c|}{58} &
  \multicolumn{1}{c|}{63.1} &
  \multicolumn{1}{c|}{62.94} &
  61.73 \\ \cline{2-8} 
\multicolumn{1}{c|}{} &
  BL2 FedEraser &
  \multicolumn{1}{c|}{84.03} &
  \multicolumn{1}{c|}{35.01} &
  \multicolumn{1}{c|}{76.74} &
  \multicolumn{1}{c|}{75.8} &
  \multicolumn{1}{c|}{79.05} &
  82.49 \\ \cline{2-8} 
\multicolumn{1}{c|}{} &
  BL3 Increase Loss &
  \multicolumn{1}{c|}{87.83} &
  \multicolumn{1}{c|}{43.53} &
  \multicolumn{1}{c|}{80.29} &
  \multicolumn{1}{c|}{81.6} &
  \multicolumn{1}{c|}{83.4} &
  85.74 \\ \cline{2-8} 
\multicolumn{1}{c|}{} &
  Bl4 Class Pruning &
  \multicolumn{1}{c|}{89.16} &
  \multicolumn{1}{c|}{39.42} &
  \multicolumn{1}{c|}{81.1} &
  \multicolumn{1}{c|}{78.2} &
  \multicolumn{1}{c|}{82.99} &
  88.09 \\ \hline
\multicolumn{1}{c|}{\multirow{5}{*}{\textbf{Painting}}} &
  BL0 Retrain &
  \multicolumn{1}{c|}{85.17} &
  \multicolumn{1}{c|}{45.21} &
  \multicolumn{1}{c|}{69.79} &
  \multicolumn{1}{c|}{75.9} &
  \multicolumn{1}{c|}{80.77} &
  81.23 \\ \cline{2-8} 
\multicolumn{1}{c|}{} &
  BL1 Repaid Retrain &
  \multicolumn{1}{c|}{71.1} &
  \multicolumn{1}{c|}{33.64} &
  \multicolumn{1}{c|}{47.5} &
  \multicolumn{1}{c|}{66.4} &
  \multicolumn{1}{c|}{63.93} &
  58.3 \\ \cline{2-8} 
\multicolumn{1}{c|}{} &
  BL2 FedEraser &
  \multicolumn{1}{c|}{84.79} &
  \multicolumn{1}{c|}{43.68} &
  \multicolumn{1}{c|}{70.11} &
  \multicolumn{1}{c|}{72.9} &
  \multicolumn{1}{c|}{76.99} &
  79.96 \\ \cline{2-8} 
\multicolumn{1}{c|}{} &
  BL3 Increase Loss &
  \multicolumn{1}{c|}{87.07} &
  \multicolumn{1}{c|}{46.42} &
  \multicolumn{1}{c|}{74.47} &
  \multicolumn{1}{c|}{81.3} &
  \multicolumn{1}{c|}{81.76} &
  85.56 \\ \cline{2-8} 
\multicolumn{1}{c|}{} &
  Bl4 Class Pruning &
  \multicolumn{1}{c|}{87.64} &
  \multicolumn{1}{c|}{46.58} &
  \multicolumn{1}{c|}{71.73} &
  \multicolumn{1}{c|}{75.9} &
  \multicolumn{1}{c|}{80.61} &
  85.38 \\ \hline
\multicolumn{1}{c|}{\multirow{5}{*}{\textbf{Quickdraw}}} &
  BL0 Retrain &
  \multicolumn{1}{c|}{84.98} &
  \multicolumn{1}{c|}{47.03} &
  \multicolumn{1}{c|}{81.1} &
  \multicolumn{1}{c|}{51.7} &
  \multicolumn{1}{c|}{82.83} &
  84.12 \\ \cline{2-8} 
\multicolumn{1}{c|}{} &
  BL1 Repaid Retrain &
  \multicolumn{1}{c|}{69.39} &
  \multicolumn{1}{c|}{34.7} &
  \multicolumn{1}{c|}{62.84} &
  \multicolumn{1}{c|}{41} &
  \multicolumn{1}{c|}{71.82} &
  59.93 \\ \cline{2-8} 
\multicolumn{1}{c|}{} &
  BL2 FedEraser &
  \multicolumn{1}{c|}{81.18} &
  \multicolumn{1}{c|}{42.62} &
  \multicolumn{1}{c|}{76.74} &
  \multicolumn{1}{c|}{48.80} &
  \multicolumn{1}{c|}{76.17} &
  77.62 \\ \cline{2-8} 
\multicolumn{1}{c|}{} &
  BL3 Increase Loss &
  \multicolumn{1}{c|}{83.27} &
  \multicolumn{1}{c|}{47.95} &
  \multicolumn{1}{c|}{77.38} &
  \multicolumn{1}{c|}{55.1} &
  \multicolumn{1}{c|}{78.88} &
  80.87 \\ \cline{2-8} 
\multicolumn{1}{c|}{} &
  Bl4 Class Pruning &
  \multicolumn{1}{c|}{86.69} &
  \multicolumn{1}{c|}{49.47} &
  \multicolumn{1}{c|}{83.36} &
  \multicolumn{1}{c|}{56.2} &
  \multicolumn{1}{c|}{82.91} &
  86.82 \\ \hline
\multicolumn{1}{c|}{\multirow{5}{*}{\textbf{Real}}} &
  BL0 Retrain &
  \multicolumn{1}{c|}{85.55} &
  \multicolumn{1}{c|}{45.81} &
  \multicolumn{1}{c|}{75.28} &
  \multicolumn{1}{c|}{76.4} &
  \multicolumn{1}{c|}{71.98} &
  86.1 \\ \cline{2-8} 
\multicolumn{1}{c|}{} &
  BL1 Repaid Retrain &
  \multicolumn{1}{c|}{71.67} &
  \multicolumn{1}{c|}{32.42} &
  \multicolumn{1}{c|}{53.63} &
  \multicolumn{1}{c|}{70.4} &
  \multicolumn{1}{c|}{54.89} &
  56.86 \\ \cline{2-8} 
\multicolumn{1}{c|}{} &
  BL2 FedEraser &
  \multicolumn{1}{c|}{83.84} &
  \multicolumn{1}{c|}{42.62} &
  \multicolumn{1}{c|}{74.64} &
  \multicolumn{1}{c|}{71.30} &
  \multicolumn{1}{c|}{70.99} &
  81.41 \\ \cline{2-8} 
\multicolumn{1}{c|}{} &
  BL3 Increase Loss &
  \multicolumn{1}{c|}{84.6} &
  \multicolumn{1}{c|}{43.07} &
  \multicolumn{1}{c|}{76.74} &
  \multicolumn{1}{c|}{77.2} &
  \multicolumn{1}{c|}{75.76} &
  84.48 \\ \cline{2-8} 
\multicolumn{1}{c|}{} &
  Bl4 Class Pruning &
  \multicolumn{1}{c|}{84.98} &
  \multicolumn{1}{c|}{47.64} &
  \multicolumn{1}{c|}{78.03} &
  \multicolumn{1}{c|}{79.2} &
  \multicolumn{1}{c|}{72.97} &
  87.36 \\ \hline
\multicolumn{1}{c|}{\multirow{5}{*}{\textbf{Sketch}}} &
  BL0 Retrain &
  \multicolumn{1}{c|}{81.56} &
  \multicolumn{1}{c|}{43.99} &
  \multicolumn{1}{c|}{75.28} &
  \multicolumn{1}{c|}{70.5} &
  \multicolumn{1}{c|}{78.8} &
  66.43 \\ \cline{2-8} 
\multicolumn{1}{c|}{} &
  BL1 Repaid Retrain &
  \multicolumn{1}{c|}{65.59} &
  \multicolumn{1}{c|}{30.44} &
  \multicolumn{1}{c|}{52.83} &
  \multicolumn{1}{c|}{63.40} &
  \multicolumn{1}{c|}{59.98} &
  40.61 \\ \cline{2-8} 
\multicolumn{1}{c|}{} &
  BL2 FedEraser &
  \multicolumn{1}{c|}{77.57} &
  \multicolumn{1}{c|}{42.62} &
  \multicolumn{1}{c|}{72.21} &
  \multicolumn{1}{c|}{68.00} &
  \multicolumn{1}{c|}{73.54} &
  64.44 \\ \cline{2-8} 
\multicolumn{1}{c|}{} &
  BL3 Increase Loss &
  \multicolumn{1}{c|}{86.69} &
  \multicolumn{1}{c|}{49.47} &
  \multicolumn{1}{c|}{81.1} &
  \multicolumn{1}{c|}{78.1} &
  \multicolumn{1}{c|}{80.36} &
  81.41 \\ \cline{2-8} 
\multicolumn{1}{c|}{} &
  Bl4 Class Pruning &
  \multicolumn{1}{c|}{84.6} &
  \multicolumn{1}{c|}{47.95} &
  \multicolumn{1}{c|}{78.19} &
  \multicolumn{1}{c|}{73.4} &
  \multicolumn{1}{c|}{80.03} &
  78.16 \\% \hline
\end{tabular}
\end{table*}

==> Office10_test_acc.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\begin{tabular}{cl|cccc}
%\hline
\multicolumn{2}{c|}{\multirow{2}{*}{\textbf{Office-Caltech10}}} &
  \multicolumn{4}{c}{\multirow{2}{*}{Test  ACC  For All  Domain}} \\
\multicolumn{2}{c|}{} &
  \multicolumn{4}{c}{} \\ \hline
\multicolumn{1}{c|}{\textbf{Unlearn Domain}} &
  \textbf{BaseLine} &
  \multicolumn{1}{c|}{\textbf{Amazon}} &
  \multicolumn{1}{c|}{\textbf{Caltech}} &
  \multicolumn{1}{c|}{\textbf{Dslr}} &
  \textbf{Webcam} \\ \hline
\multicolumn{1}{c|}{\textbf{/}} &
  Full learn &
  \multicolumn{1}{c|}{78.12} &
  \multicolumn{1}{c|}{76} &
  \multicolumn{1}{c|}{90.62} &
  89.83 \\ \hline
\multicolumn{1}{c|}{\multirow{5}{*}{\textbf{Amazon}}} &
  BL0 Retrain &
  \multicolumn{1}{c|}{64.38±1.63} &
  \multicolumn{1}{c|}{70.67±1.61} &
  \multicolumn{1}{c|}{86.25±5.08} &
  88.81±3.32 \\ \cline{2-6} 
\multicolumn{1}{c|}{} &
  BL1 Repaid Retrain &
  \multicolumn{1}{c|}{46.25±2.90} &
  \multicolumn{1}{c|}{52.27±1.55} &
  \multicolumn{1}{c|}{82.50±3.75} &
  94.92±1.86 \\ \cline{2-6} 
\multicolumn{1}{c|}{} &
  BL2 FedEraser &
  \multicolumn{1}{c|}{53.26±5.72} &
  \multicolumn{1}{c|}{59.22±1.61} &
  \multicolumn{1}{c|}{83.59±5.12} &
  83.05±1.20 \\ \cline{2-6} 
\multicolumn{1}{c|}{} &
  BL3 Increase Loss &
  \multicolumn{1}{c|}{73.23±0.42} &
  \multicolumn{1}{c|}{74.49±0.72} &
  \multicolumn{1}{c|}{88.75±2.50} &
  89.83±1.07 \\ \cline{2-6} 
\multicolumn{1}{c|}{} &
  Bl4 Class Pruning &
  \multicolumn{1}{c|}{67.40±1.50} &
  \multicolumn{1}{c|}{68.80±1.10} &
  \multicolumn{1}{c|}{90.00±4.15} &
  87.12±3.14 \\ \hline
\multicolumn{1}{c|}{\multirow{5}{*}{\textbf{Caltehc}}} &
  BL0 Retrain &
  \multicolumn{1}{c|}{35.42±2.19} &
  \multicolumn{1}{c|}{34.13±2.41} &
  \multicolumn{1}{c|}{75.00±1.98} &
  91.86±3.29 \\ \cline{2-6} 
\multicolumn{1}{c|}{} &
  BL1 Repaid Retrain &
  \multicolumn{1}{c|}{35.62±1.53} &
  \multicolumn{1}{c|}{32.09±1.17} &
  \multicolumn{1}{c|}{70.62±4.24} &
  92.20±1.73 \\ \cline{2-6} 
\multicolumn{1}{c|}{} &
  BL2 FedEraser &
  \multicolumn{1}{c|}{57.03±8.59} &
  \multicolumn{1}{c|}{37.56±3.33} &
  \multicolumn{1}{c|}{65.62±3.12} &
  84.75±5.08 \\ \cline{2-6} 
\multicolumn{1}{c|}{} &
  BL3 Increase Loss &
  \multicolumn{1}{c|}{80.73±0.66} &
  \multicolumn{1}{c|}{69.87±0.33} &
  \multicolumn{1}{c|}{76.88±1.53} &
  86.78±0.68 \\ \cline{2-6} 
\multicolumn{1}{c|}{} &
  Bl4 Class Pruning &
  \multicolumn{1}{c|}{49.27±5.26} &
  \multicolumn{1}{c|}{47.02±3.10} &
  \multicolumn{1}{c|}{78.12±5.59} &
  94.92±2.40 \\ \hline
\multicolumn{1}{c|}{\multirow{5}{*}{\textbf{Dslr}}} &
  BL0 Retrain &
  \multicolumn{1}{c|}{81.04±4.11} &
  \multicolumn{1}{c|}{74.31±2.29} &
  \multicolumn{1}{c|}{76.88±7.55} &
  89.49±4.21 \\ \cline{2-6} 
\multicolumn{1}{c|}{} &
  BL1 Repaid Retrain &
  \multicolumn{1}{c|}{74.58±1.45} &
  \multicolumn{1}{c|}{62.04±1.88} &
  \multicolumn{1}{c|}{72.50±4.15} &
  85.08±3.92 \\ \cline{2-6} 
\multicolumn{1}{c|}{} &
  BL2 FedEraser &
  \multicolumn{1}{c|}{74.35±5.97} &
  \multicolumn{1}{c|}{70.44±2.36} &
  \multicolumn{1}{c|}{66.41±8.08} &
  75.42±6.62 \\ \cline{2-6} 
\multicolumn{1}{c|}{} &
  BL3 Increase Loss &
  \multicolumn{1}{c|}{82.40±1.52} &
  \multicolumn{1}{c|}{74.22±1.01} &
  \multicolumn{1}{c|}{80.62±6.67} &
  82.03±2.96 \\ \cline{2-6} 
\multicolumn{1}{c|}{} &
  Bl4 Class Pruning &
  \multicolumn{1}{c|}{82.60±1.88} &
  \multicolumn{1}{c|}{75.56±1.12} &
  \multicolumn{1}{c|}{80.00±3.75} &
  88.14±4.01 \\ \hline
\multicolumn{1}{c|}{\multirow{5}{*}{\textbf{Webcam}}} &
  BL0 Retrain &
  \multicolumn{1}{c|}{78.65±1.10} &
  \multicolumn{1}{c|}{74.78±1.38} &
  \multicolumn{1}{c|}{79.69±5.18} &
  69.92±5.00 \\ \cline{2-6} 
\multicolumn{1}{c|}{} &
  BL1 Repaid Retrain &
  \multicolumn{1}{c|}{70.73±3.43} &
  \multicolumn{1}{c|}{62.40±1.24} &
  \multicolumn{1}{c|}{77.50±3.64} &
  71.19±3.22 \\ \cline{2-6} 
\multicolumn{1}{c|}{} &
  BL2 FedEraser &
  \multicolumn{1}{c|}{76.04±3.01} &
  \multicolumn{1}{c|}{69.33±3.89} &
  \multicolumn{1}{c|}{69.53±11.56} &
  55.51±2.51 \\ \cline{2-6} 
\multicolumn{1}{c|}{} &
  BL3 Increase Loss &
  \multicolumn{1}{c|}{82.92±1.37} &
  \multicolumn{1}{c|}{74.13±1.67} &
  \multicolumn{1}{c|}{81.88±1.25} &
  69.83±2.25 \\ \cline{2-6} 
\multicolumn{1}{c|}{} &
  Bl4 Class Pruning &
  \multicolumn{1}{c|}{76.35±5.31} &
  \multicolumn{1}{c|}{73.78±1.84} &
  \multicolumn{1}{c|}{80.00±4.24} &
  65.76±10.02 \\% \hline
\end{tabular}
\end{table*}

==> differenet_setting_test.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[!h]
\begin{tabular}{ccccccc}
\hline
\multirow{2}{*}{Domain} & \textbf{Setting} & \multicolumn{5}{c}{\textbf{Test  ACC  For All  Domain}} \\
                       & \textbf{eps/poison} & MNIST & SVHN  & USPS  & SynthDigits & MNIST-M \\ \hline
/                      & \textbf{Clean}      & 98.91 & 83.36 & 97.42 & 93.57       & 90.40   \\ \hline
\multirow{5}{*}{MNIST} & \textbf{0.3/0.5}    & 98.91 & 82.30 & 97.90 & 94.73       & 92.72   \\
                       & \textbf{0.1/0.5}    & 98.96 & 84.22 & 98.12 & 94.61       & 90.64   \\
                       & \textbf{0.6/0.5}    & 98.86 & 84.14 & 97.90 & 94.61       & 92.59   \\
                       & \textbf{0.3/0.7}    & 98.83 & 83.99 & 98.01 & 94.83       & 92.60   \\
                       & \textbf{0.3/0.3}    & 98.80 & 83.93 & 98.06 & 94.87       & 92.48   \\ \hline
\multirow{5}{*}{SVHN}  & \textbf{0.3/0.5}    & 98.89 & 98.89 & 98.33 & 93.68       & 91.36   \\
                       & \textbf{0.1/0.5}    & 98.91 & 80.62 & 97.69 & 94.42       & 92.84   \\
                       & \textbf{0.6/0.5}    & 98.89 & 82.9  & 98.06 & 94.87       & 92.17   \\
                       & \textbf{0.3/0.7}    & 99.07 & 80.21 & 98.12 & 94.12       & 92.94   \\ 
                       & \textbf{0.3/0.3}    & 99.03 & 82.43 & 97.9  & 94.25       & 92.57  \\ \hline
\end{tabular}
\end{table}

==> differenet_setting_train.tex <==

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[!h]
\begin{tabular}{ccccccc}
\hline
\multirow{2}{*}{Doamin}  & \multirow{2}{*}{Method} & \multicolumn{5}{c}{\multirow{2}{*}{\textbf{Train ACC  For BaseLine}}} \\  
                        &          & \multicolumn{5}{c}{}                    \\ \hline
/                       & /        & Retrain & BL1   & BL2   & BL3   & BL4   \\ \hline
\multirow{3}{*}{Amzon}  & Clean    & 64.38   & 46.25 & 53.26 & 73.23 & 67.4  \\
                        & Backdoor & 0       & 0     & 0     & 0     & 0     \\
                        & Ours     & 0       & 0     & 0     & 6.65  & 7.44  \\ \hline
\multirow{3}{*}{Caltech} & Clean                   & 34.13       & 32.09       & 37.56      & 69.87      & 47.02      \\
                        & Backdoor & 0       & 0     & 0     & 0     & 0     \\
                        & Ours     & 0       & 0     & 0     & 17.59 & 21.27 \\\hline
\multirow{3}{*}{Dslr}   & Clean    & 76.88   & 72.5  & 66.41 & 80.62 & 80    \\
                        & Backdoor & 0       & 0     & 0     & 0     & 0     \\
                        & Ours     & 0       & 0     & 0     & 9.3   & 6.12  \\ \hline
\multirow{3}{*}{Webcam} & Clean    & 69.92   & 71.19 & 55.51 & 69.83 & 73.22 \\
                        & Backdoor & 0       & 0     & 0     & 0     & 0     \\
                        & Ours     & 0       & 0     & 0     & 32.21 & 23.73 \\ \hline
\end{tabular}
\end{table}








% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \begin{table}[]
% \begin{tabular}{cccccccc}
% \hline
% \multirow{2}{*}{Domain} & \multirow{2}{*}{\textbf{Setting}} & \multicolumn{6}{c}{\multirow{2}{*}{\textbf{Train ACC  For BaseLine}}} \\  
%                        &                     & \multicolumn{6}{c}{}                            \\ \hline
% /                      & \textbf{eps/poison} & Full  & Retrain & BL1   & BL2   & BL3   & BL4   \\ \hline
% \multirow{5}{*}{MNIST} & \textbf{0.3/0.5}    & 99.93 & 50.87   & 51.53 & 61.13 & 93.47 & 70.49 \\
%                        & \textbf{0.1/0.5}    & 10.84 & 10.86   & 11.27 & 12.60 & 11.66 & 11.13 \\
%                        & \textbf{0.6/0.5}    & 94.54 & 15.97   & 24.74 & 16.38 & 78.21 & 24.28 \\
%                        & \textbf{0.3/0.7}    & 99.83 & 52.50   & 51.17 & 70.96 & 96.50 & 66.83 \\
%                        & \textbf{0.3/0.3}    & 99.62 & 52.50   & 51.17 & 73.65 & 97.88 & 75.36 \\ \hline
% \multirow{5}{*}{SVHN}  & \textbf{0.3/0.5}    & 95.90 & 71.83   & 65.80 & 78.02 & 83.46 & 82.90 \\
%                        & \textbf{0.1/0.5}    & 75.14 & 53.70   & 46.42 & 66.85 & 55.45 & 60.58 \\
%                        & \textbf{0.6/0.5}    & 99.19 & 68.14   & 52.07 & 74.91 & 42.48 & 62.84 \\
%                        & \textbf{0.3/0.7}    & 94.73 & 71.83   & 65.80 & 84.01 & 70.17 & 74.31 \\
%                        & \textbf{0.3/0.3}    & 98.82 & 71.83   & 65.80 & 76.77 & 84.47 & 62.99 \\ \hline
% \end{tabular}
% \end{table}
